Technical Report: On the Convergence of Gossip Learning in the Presence of Node Inaccessibility

Gossip learning (GL), as a decentralized alternative to federated learning (FL), is more suitable for resource-constrained wireless networks, such as Flying Ad-Hoc Networks (FANETs) that are formed by unmanned aerial vehicles (UAVs). GL can significantly enhance the efficiency and extend the battery life of UAV networks. Despite the advantages, the performance of GL is strongly affected by data distribution, communication speed, and network connectivity. However, how these factors influence the GL convergence is still unclear. Existing work studied the convergence of GL based on a virtual quantity for the sake of convenience, which failed to reflect the real state of the network when some nodes are inaccessible. In this paper, we formulate and investigate the impact of inaccessible nodes to GL under a dynamic network topology. We first decompose the weight divergence by whether the node is accessible or not. Then, we investigate the GL convergence under the dynamic of node accessibility and theoretically provide how the number of inaccessible nodes, data non-i.i.d.-ness, and duration of inaccessibility affect the convergence. Extensive experiments are carried out in practical settings to comprehensively verify the correctness of our theoretical findings.

==> useless.tex <==
\subsection{Blockchain-Enabled Decentralized Federated Learning}
One branch of work introduce edge server, where the aggregation in federated leaning can be performed in a hierarchical way. However, crisis of confidence is not resolved since it does not eliminate the possibility that an edge server can be compromised. 
The other branch of research utilize blockchain as public ledger to record the whole learning trace and perform automatic aggregation by smart contract. If abnormal/malicious behavior in training process is detected, one can trace back the error step and restore the model. Blockchain could also identify the malicious identity by the tractability and anti-tamper property. However, in FL paradigm, the blockchain needs to store all model parameter from all participants and each participants needs to run \textcolor{red}{consensus}? Such frequent interaction and synchronization between vehicles and blockchain consume xx computation and storage, causing the efficiency too low. 
In addition, blockchain-based decentralizaed learning still has the sense of a "global model" that is aggregated from training participants, and the nodes still need to synchronize such a global model. 

To achieve this goal, each node runs SGD on its local data $D_k$ to optimize its local model $w_k$. For convenience, we assume that each node possesses the same mount of data.
Then, the aggregation operation on the FL server can be formulated as:
\begin{align}
    w^{T+1} \leftarrow \frac{1}{K} \sum_{k=1}^K w_k^{T
}\\
  w^{T+1} \leftarrow w^T + \frac{\eta}{K} \sum_{k=1}^K \Delta w_k^{T}
\end{align}

Suppose node $k$' clock is ticked by $t_k$. Then, node $k$ trains the local model $w_k$ on its own data $D_k$ and update the local model. Node $k$ then broadcasts its local model to one of its neighbor nodes. Once the local is received, the neighboring node merges the received model with its own local model.

It has been empirically shown that gossip learning outperforms FL under the same amount communication and compression. However, since it is an opportunistic algorithm, it is not guaranteed that it always achieve the best performance/convergence.

\subsection{Aggregation}
The most popular aggregation algorithm is FedAvg\cite{mcmahan2017communication}, which is an average algorithm weighted by the amount of data on which each local model was trained. 
\begin{align}
    w^{T+1} = \sum_{k=1}^K \frac{n_k}{n} \Delta w_k^T,
\end{align}
where $T$ is the global training epoch, $n_k = D_k$ is the number of training data for local model $w_k$
 and $n=\sum_{k=1}^K n_k$ is the total number of training data. 
However, due to the non-i.i.d. data distribution among participating users, and multiple SGDs are performed on each sub-area could introduce weight divergence \cite{zhao2018federated}, i.e. the trained models in each sub-area may be different from others, which degrades/neutralize the global model performance when aggregated.

\section{Our Design}
Here, we strictly define that each node communicate with no more than one neighbor in each time slot/training step.
\subsection{Consensus}
At time $t$, each node $k$ has an estimate of the global model. 
The average consensus is to make all nodes in the network reach the consistent state of the average of the initial states $X_i$, which is formally defined as the following formula:
\begin{align}
   \Bar{X}:= \frac{1}{n}\sum_{i=1}^n X_i 
\end{align}
In gossip learning, a
The aggregation operation in the federated learning


\begin{algorithm}
\caption{The Proposed Gossip Learning Algorithm}\label{alg::gossip}
\begin{algorithmic}[1]
% \renewcommand{\algorithmicwhile}{\textbf{loop}} 
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
\State $(t_k, w_k) \leftarrow $init()
\Loop
\State wait($\Delta_g)$
\State $p \leftarrow$ select()
\State send ($t_k$, compress($w_k$)) to $p$
\EndLoop
\Procedure {\textsc{On}\textsc{Receive}\textsc{Model}} {$t_r, w_r$}
\State {($t_k, w_k$) $\leftarrow$ merge($(t_k, w_k), (t_r, w_r)$)}
\State ($t_k, w_k$) $\leftarrow$ update(($t_k, w_k), D_k$)
\EndProcedure
\end{algorithmic}
\end{algorithm}


Conventional GL assumes the gossip matrix to be a doubly stochastic matrix, which has the averaging property. This assumption guarantees the consensus when the gossip objective is trivial, i.e., simple message synchronization, linear regression or computing the average. 


Realizing the deficiency and inability of central server in ad-hoc like dynamic network topology, in this paper, we propose a novel fully decentralized learning framework, where gossip protocol adapts the collaborative learning to ad-hoc dynamic networks, while blockchain serves helps in getting rid of all kinds of server and realizing fully decentralization. The proposed decentralized learning framework makes the collaborative learning task more practical and applicable to general ad-hoc networks. 


Note that this quantity is not available to the workers at any given time, but it will be conveniently to use for the proofs.


The data on such vehicles includes the driving habits, maintaining history, current location, destination, driving routes and etc.. Performing data mining on such data is of high interest, which could help the service provider improve the service quality, safety, and user/driver experience. 
However directly releasing the data could disclose users privacy, in the worst case could pose threats to drivers' lives. 

\textbf{(3) Inability to reliability issue. }
% Due to the distributed nature and inherent data non-i.i.d-ness across electric vehicles/drones, the uploaded model parameter by one user may be different from others. Although the central server collects the model parameter from all users, there is still little can be done by central server to validate their legitimacy/truthfulness. 



 
% Despite the sensors on vehicles and drones, the newly added sensors that enables intelligent applications, such as camera, mmWave, LiDAR and GPS, would generated huge amount of data. The large number of participants and the complex model  
could further deteriorate the learning efficiency.



However, the limitation of gossip learning protocol lies in the fully distributed data model, the requirement for full connectivity and the assumption of homogeneous communications speeds \cite{giaretta2019gossip}.

% FL in MANET 存在困难。
Federated learning (FL) serves as a solution that utilizes the data generated/collected distributively to train a machine learning models that enables intelligent agricultural applications, while enjoying the benefits of efficient communication (transmitting parameters instead of raw data). However, the deployment of FL on UAVs faces difficulties. 
% 1. power consumption。
\textbf{(1) Power consumption.} FL framework requires one central to coordinate the whole training process, including the selection of participants, global model synchronization, model parameter collection and aggregation. The server could be remote or played by one of the drones. In the former solution, each node would need increase power to reach the base station, which reduces the battery life. 
% 2. 拓扑迅速变化。routing困难？


% 3. 单点失败。影响效率，影响收敛。ad-hoc没有collison resistance? 
\textbf{(5) Single point failure.} 




 Nodes reach consensus $\bar{w}^{t+1}$ in the asymptotic time limit ($T\rightarrow \infty$). Define $w^t:= [w_1^t,...,w_n^t]$.
% $\mathbf{\bar{W}}^t:= [w_1^t,...,w_n^t]$
\begin{small} \begin{flalign}
\dot{w}^{t+1} = A(w^{T+\frac{1}{2}} ).
\end{flalign}\end{small}

 \sum_{k \in \mathcal{S} \backslash \mathcal{S}_{in}^T} A_i^T w_i^T),

 \begin{small} \begin{align}
A_1 &= -\frac{2\eta}{tn_1} (f(w^T) - f(w^*)) - \frac{\mu\eta}{2 n_1}\sum_{i, t} \|w^T - w^*\| \nonumber \\
+ &\frac{2L\eta}{tn_1}\|w_i^{T-\tau(T, i), \tau} - w^T\|
\end{align}\end{small}

\begin{small} \begin{align}
&w_i^{T-\tau(T, i), \tau} - w^T \nonumber \\
=& w_i^{T-\tau(T, i), \tau} - w^{T-\tau(T, i)} + w^{T-\tau(T, i)} - w^T \nonumber\\
=& w_i^{T-\tau(T, i), \tau} - w^{T-\tau(T, i)} - \frac{\eta}{n_1} \sum_{j=T-\tau(T, i)}^{T}\sum_{i=1}^{n_1}\nabla f_i(w^{j-\tau{j, i}})
\end{align}\end{small}


\begin{small} \begin{align}
\|w_i^{T-\tau(T, i), \tau} - w^T\| &\leq 2\| w_i^{T-\tau(T, i), \tau} - w^{T-\tau(T, i)}\| \nonumber \\
+& 2\|\frac{\eta}{n_1} \sum_{j=T-\tau(T, i)}^{T}\sum_{i=1}^{n_1}\nabla f_i(w^{j-\tau{j, i}}) \|
\end{align}\end{small}

% \begin{small}\begin{flalign}
%     A_1 = & 2\big[\langle  w^*- w^{T, k}  + w^{T, k} - {w}^{T}, \frac{1}{n_1}\sum_{i=1}^{n_1} \nabla f(\bar{w}^T,\xi_i) \rangle\big]\nonumber \\
%     =& \frac{2\eta }{n_1} \sum_{i=1}^{n_1} \sum_{k=0}^t\big[\langle w^*- w^T  + w^{T,k} -w^{T,k} , \nabla f(\bar{w}^{T,k},\xi_i)\rangle\big] \nonumber\\
%     =& \underbrace{ \frac{2\eta}{n_1} \sum_{i=1}^{n_1} \sum_{k=0}^t \big[\langle {w}^{T,k} -w^T , \nabla f(\bar{w}^{T,k}, \xi_i )\rangle\big]}_{B_3} \nonumber\\ 
%     &+  \underbrace{\frac{2\eta t}{n_2} \sum_{i=1}^{n_2}\sum_{k=0}^t \big[\langle  w^* - {w}^{T,k} , \nabla f(\bar{w}^{T,k}, \xi_i )\rangle\big]}_{B_4}
% \end{flalign}\end{small}


% \begin{small}\begin{flalign}
%     B_3& \leq  \frac{1}{n_1} \sum_{i=1}^{n_1} \sum_{k=0}^t \big[\| {w}^{T,k} -w^T \| +  \frac{\eta^2}{n_1} \sum_{i=1}^{n_1} \sum_{k=0}^t\|\nabla f(\bar{w}^{T,k}, \xi_i )\|\big] \nonumber \\
%     \leq &  \frac{1}{n_1}\sum_{i=1}^{n_1} \sum_{k=0}^t   \bigg[ \big\|\nabla f({w}^{T, k}, \xi_i)\big\|^2\bigg]  +\frac{\eta^2 } {n_1} \sum_{i=1}^{n_2}   \big[\|\nabla f(\bar{w}_i^{T,k}, \xi_i\|^2\big]
%       % \leq & \frac{ \tau(T, i) (\tau(T, i)+1)(2\tau(T, i)+1)t \eta^2 G^2}{6} + \tau(T, i)\eta^2 t G^2,
% \end{flalign}\end{small}

% \begin{small}\begin{flalign}
%     B_4&  \overset{(a)} \leq -\frac{2\eta t}{n_2} \sum_{i=1}^{n_2}\sum_{k=0}^t \big[\langle  w^* - \bar{w}^{T,k} , \nabla f(\bar{w}^{T,k}, \xi_i )\rangle\big] \nonumber \\
%     \overset{(b)} \leq &-\frac{2 \eta t}{n_1}  \sum_{i \in \mathcal{A(T)}} \big[ f(w^*)- f(\bar{w}^{T,\tau}) - \frac{\mu}{2} \|\bar{w}^{T,\tau} - w^*\|^2 \big] 
%     % \leq & -\frac{2 \eta t}{n_1} 
%     %  \leq &\frac{2 \eta t}{n_2} \sum_{i \in \mathcal{A(T)}}\big[ F_i(w^*) - F_i^* + F_i^* - F_i({w}_i^{T-\tau(T, i)}) - \frac{\mu}{2} \|{w}_i^{T-\tau(T, i)} - w^*\|^2 \big] \nonumber\\
%     %  = &2 \eta t (F^* - \frac{1}{n_2}\sum_{i \in \mathcal{A(T)}} F_i^*) + \frac{2 \eta}{n_2} \sum_{i \in \mathcal{A(T)}}  (F_i^* - F_i({w}_i^{T-\tau(T, i)} )\nonumber\\
%     %  & - \frac{\mu\eta}{n} \sum_{i \in \mathcal{A(T)}}  \big[\|{w}_i^{T- \tau(T, i)} - w^*\|^2\big] \nonumber\\
%     %  \overset{(c)} \leq & 2\eta t \Gamma - \frac{\mu\eta}{n_2} \sum_{j=T-\tau(T, i)}^{T-1} \sum_{i \notin \mathcal{A(T)}}   \underbrace{\big[\|{w}_i^{j- \tau(j, i)} - w^*\|^2}_{C}\big],
% \end{flalign}\end{small}



\subsection{Proof of Theorem 1}
\label{proof_convergence_rate_convex}
\begin{proof}

Assuming that $w^*$ is the optimal parameter, $F_i^*$ and $F^*$ denote the optimal of local and global objective value. We employ the following notations of stacked vectors:
\begin{small} \begin{flalign}
w:= [w_1,...,w_n] ,~~ \nabla F(w):= [\nabla F_1(w_1),...,\nabla F_n(w_n) ].
\end{flalign}\end{small}
Since 
\begin{small} \begin{flalign}
    \bar{w}^{T+1} = \frac{1}{n}\sum_{i=1}^n [(A_i^{T})^k(w_i^{(T)}) - \frac{1}{n} \sum_{i=1}^n \Delta w_i^{(T)})], 
\end{flalign}\end{small}
where $    \Delta w_i^T = \eta \sum_{\tau=0}^{t-1}\nabla F_i(\bar{w}^{T, \tau}, \xi_i^{T, \tau}).$ 
We have the following
\begin{small}\begin{flalign}
\label{1}  
&\mathbb{E} \big[\ \|\bar{w}^{T+1} - w^*\|^2\big] = \mathbb{E} \big[\ \|\bar{w}^{T} - \frac{1}{n} \sum_{i=1}^n  \Delta w_i^T- w^*\|^2\big]
\nonumber \\= &\mathbb{E} \big[ \|\bar{w}^{T} - w^*\|^2\big] + \underbrace{\mathbb{E}\big[\|\frac{1}{n} \sum_{i=1}^n \Delta w_i^T\|^2 \big]}_{A_1}  \nonumber\\&  \underbrace{-2\mathbb{E}\big[\langle \bar{w}^T - w^*, \frac{1}{n}\sum_{i=1}^n \nabla F_i(w_i^{T})\rangle\big]}_{A_2}
\end{flalign}\end{small} 
Next, we bound the terms $A_1$ and $A_2$.

\begin{small}\begin{flalign}
    A_1 &= \mathbb{E}\big[\|\frac{1}{n}\sum_{i=1}^n \nabla F_i(w_i^{T}) \|^2\big] \leq \frac{1}{n}\sum_{i=1}^n \mathbb{E}\big[\|\nabla F_i(w_i^{T})\|^2 \big] \nonumber\\
    &=\frac{\eta^2}{n}\sum_{i=1}^n \mathbb{E}\big[\| \sum_{\tau=1}^{t-1} \nabla F_i(w^{T,\tau}_{i}, \xi^{T,\tau}_i) \|^2\big] \nonumber \\
    & \leq \frac{\eta^2t}{n} \sum_{\tau=0}^{t-1} \sum_{i=1}^n \mathbb{E}\big[\| \nabla F_i(w^{T,\tau}_{i}, \xi^{T,\tau}_i) \|^2\big] \leq \eta^2 t^2 G^2 
\end{flalign}\end{small} 

\begin{small}\begin{flalign}
    A_2 = & 2\mathbb{E}\big[\langle  w^*- \bar{w}^T  + w^{T, \tau} -w^{T, \tau}, \frac{1}{n}\sum_{i=1}^n \nabla F_i(w_i^{T} \rangle\big]\nonumber \\=& 2 \eta \sum_{i=1}^n \sum_{\tau=0}^{t-1}  \frac{1}{n} \mathbb{E}\big[\langle w^*- \bar{w}^T  + w^{T, \tau} -w^{T, \tau} , \nabla F_i({w}_i^{T, \tau}, \xi_i^{T, \tau} )\rangle\big] \nonumber\\
     =& \underbrace{ \frac{2\eta}{n} \sum_{i=1}^n \sum_{\tau=0}^{t-1}   \mathbb{E}\big[\langle {w}_i^{T, \tau} -\bar{w}^T , \nabla F_i({w}_i^{T, \tau}, \xi_i^{T, \tau} )\rangle\big]}_{B_1} \nonumber\\ &+  \underbrace{\frac{2\eta}{n} \sum_{i=1}^n \sum_{\tau=0}^{t-1}   \mathbb{E}\big[\langle  w^* - {w}_i^{T, \tau} , \nabla F_i({w}_i^{T, \tau}, \xi_i^{T, \tau} )\rangle\big]}_{B_2}
\end{flalign}\end{small}

\begin{small}\begin{flalign}
    B_1 \leq & \frac{1}{n} \sum_{i=1}^n \sum_{\tau=0}^{t-1}   \mathbb{E}\big[ \| {w}_i^{T, \tau} - \bar{w}^T \|^2\big] + \frac{\eta^2}{n} \sum_{i=1}^n \sum_{\tau=0}^{t-1}   \mathbb{E}\big[\|\nabla F_i({w}_i^{T, \tau}, \xi_i^{T, \tau}\|^2\big] \nonumber\\
    \leq &  \frac{1}{n}\sum_{i=1}^n \sum_{\tau=0}^{t-1}   \mathbb{E}\bigg[ \big\|\eta \sum_{\upsilon=0}^{\tau} \nabla F_i({w}_i^{T, \upsilon}, \xi_i^{T, \upsilon})\big\|^2\bigg] +\eta^2 t G^2 \nonumber\\
      \leq & \frac{ t (t+1)(2t+1)\eta^2 G^2}{6} + \eta^2 t G^2,
\end{flalign}\end{small}

\begin{small}\begin{flalign}
    B_2&  \overset{(a)} \leq \frac{2 \eta}{n} \sum_{i=1}^n \sum_{\tau=0}^{t-1} \mathbb{E}\big[\langle w^* -{w}_i^{T, \tau} , \nabla F_i({w}_i^{T, \tau})\rangle\big] \nonumber \\
    \overset{(b)} \leq &\frac{2 \eta}{n}  \sum_{i=1}^n \sum_{\tau=0}^{t-1}  \mathbb{E}\big[ F_i(w^*)- F_i({w}_i^{T, \tau}) - \frac{\mu}{2} \|{w}_i^{T, \tau} - w^*\|^2 \big] \nonumber\\
     \leq &\frac{2 \eta}{n} \sum_{i=1}^n \sum_{\tau=0}^{t-1}  \mathbb{E}\big[ F_i(w^*) - F_i^* + F_i^* - F_i({w}_i^{T, \tau}) - \frac{\mu}{2} \|{w}_i^{T, \tau} - w^*\|^2 \big] \nonumber\\
     = &2 \eta t (F^* - \frac{1}{n}\sum_{i=1}^n F_i^*) + \frac{2 \eta}{n} \sum_{i=1}^n \sum_{\tau=0}^{t-1} (F_i^* - F_i({w}_i^{T, \tau} )\nonumber\\
     & - \frac{\mu\eta}{n} \sum_{i=1}^n  \sum_{\tau=0}^{t-1}  \mathbb{E}\big[\|{w}_i^{T, \tau} - w^*\|^2\big] \nonumber\\
     \overset{(c)} \leq & 2\eta t \Gamma - \frac{\mu\eta}{n} \sum_{i=1}^n  \sum_{\tau=0}^{t-1}  \mathbb{E}\underbrace{\big[\|{w}_i^{T, \tau} - w^*\|^2}_{C}\big],
\end{flalign}\end{small}
where $(a)$ and $(b)$ are due to Assumptions 4 and 2, respectively. $(c)$ is by the definition of $\Gamma$, and the fact that $(F_i^* - F_i({w}_i^{T})) <0$
\begin{small}\begin{flalign}
    -C &\leq -\|{w}_i^{T, \tau} - \bar{w}^{T}\|^2 -\|\bar{w}^{T} - w^*\|^2 - 2 \langle {w}_i^{T, \tau} - \bar{w}^{T}, \bar{w}^{T} - w^*\rangle\nonumber\\
    &\leq -\|{w}_i^{T, \tau} - \bar{w}^{T}\|^2 - \|\bar{w}^{T} - w^*\|^2 + \frac{1}{\eta} \|{w}_i^{T, \tau} - \bar{w}^{T}\|^2 + \eta \|\bar{w}^{T} - w^*\|^2 \nonumber\\
    & = -(1-\eta) \|\bar{w}_i^{T} - w^*\|^2 + (\frac{1}{\eta}-1)\|{w}_i^{T, \tau} - \bar{w}^{T}\|^2,
\end{flalign}\end{small}
Substituting $A_1$, $A_2$, $B_1$, $B_2$ and $C$ to Eq. \ref{1}, we have
\begin{small}\begin{flalign}
\label{2}
    \mathbb{E} \big[\ \|\bar{w}^{t+1} - w^*\|^2\big] \leq& (1-\mu\eta t (1-\eta)) \mathbb{E} \big[\|\bar{w}^{T} - w^*\|_2^2\big] + 2 \eta t \Gamma \nonumber\\
   & + (1 +\mu(1-\eta))\eta^2 G^2\frac{ t (t+1)(2t+1) }{6} \nonumber\\
   &+ \eta^2 t G^2(t+1).
\end{flalign}\end{small}
Rearranging Eq. \ref{2} and summing from $0$ to $T$, we have proved Theorem \ref{theorem_convergence_convex}.
\end{proof}




(2) Unbalanced nodes distribution: the nodes can move in an area with two squares, whose length is $1000$ and $800$, respectively and squares has an overlapped area of $100m \times 100m$. 

When the weight divergence happens, i.e., the approximate consensus is not reached, descending individual $F_i(w_i)$ may not contribute to the descent of $F(\bar{w}_(i))$. Therefore, it is critical to understand the weight divergence $\|w_i - \bar{w}_i\|$ and the factors that could amplify this weight divergence.

Existing work analyzed the convergence of GL under the average consensus scenario, which the average is preserved in each iteration, $\bar{w}^{t+1} = \bar{w}^t$. And the subsequent  and claimed that. 
However, the variance of models, i.e., $\|w_i - \bar{w}\|^2$ is not 
represent the practical situation.


    % \item \textbf{Asynchronous:} The training is performed in a self-organized way, as the model is updated locally when each pair of neighbors share their models. In the presence of latency or link loss, the active nodes proceeds to the next iteration instead of waiting for the updates as in FL, which greatly mitigates the stale effect in FL.  
    \item \textbf{Scalability:} GL is inherently scalable, where increase the number of nodes does not increase the operations neither loads on nodes. In FL, increasing the number of nodes will overwhelms the server in both communication and memory. 
    \item \textbf{Node equivalence:} GL nodes are equivalent, with no node playing a specialized role, providing GL with system robustness/reliability. Unlike in FL, the frequent communication on the server node would quickly drain the battery of the server node. 


    % \item \textbf{Initialization.} In the $t$-th global aggregation, the central server broadcasts the latest global model $w^{t}$ to all nodes: $ w^{t, 0}_{i} \leftarrow w^{t} $. 
% \begin{small}
% \begin{flalign}
%     w^{t}_{i} \leftarrow w^{t}_{i} - \eta \nabla F_i(w^{t}_{i}),
% \end{flalign}
% \end{small}
% where $\eta$ is the local learning rate. After performing $t$ steps, the client calculates the model updates $\Delta w^{t}_{i} = w^{t}_i - w^{t}$.
% \item \textbf{Aggregation.} The central server then updates the global model by performing
% \begin{small}
% \begin{flalign}
% w^{T+1} \leftarrow  w^{T} + \sum_{i=1}^{n}  \frac{1}{n} \Delta w^{T}_{i}.
% \end{flalign}
% \end{small}
% \end{enumerate}
% \begin{enumerate}
% \setcounter{enumi}


\begin{small} \begin{flalign}
\bar{w}^{t}:= \frac{1}{n}\sum_{i\in \mathcal{S}} w_i^{t} = \frac{1}{n} \sum_{i\in \mathcal{S}} (\sum_{j\in \mathcal{S}} g_{ij}^t  w_i^t - \eta \nabla F_i(w^{t}_{i})),
\end{flalign} \end{small}


Their corresponding gradients are $\nabla F_i(\bar{w})$, $\nabla F_i(\overline{w})$ and $\nabla F_i(w_i)$. 
% 这里以什么对齐比较美观

\begin{small} \begin{flalign}
\text{For}~i \in S,~\nabla F_i(\bar{w}^t)&=  \nabla F(\bar{w}^{t}, D_i) \\
% 这里是写平均还是实际的值
% 平均
\text{For}~i \in A(t),~\nabla F_i(\widetilde{w}^t)&=  \nabla F_i(\sum_{i\in \mathcal{S}} g_{ij}^t w_i^{t}, D_i)\\
% 真实的值
\text{For}~i \in A(t),~\nabla F_i(\widetilde{w}^{t+\frac{1}{2}})&=  \nabla F_i(\sum_{i\in \mathcal{S}} g_{ij}^t w_i^{t}, D_i)\\
\text{For}~i \notin A(t),~\nabla F_i(w_i^{t+\frac{1}{2}})&=  \nabla F_i(w_i^{t}, D_i)\\
\end{flalign} \end{small}

